Differentially Private Episodic Reinforcement Learning with Heavy-tailed Rewards

In this paper, we study the problem of (finite horizon tabular) Markov decision processes (MDPs) with heavy-tailed rewards under the constraint of differential privacy (DP). Compared with the previous studies for private reinforcement learning that typically assume rewards are sampled from some bounded or sub-Gaussian distributions to ensure DP, we consider the setting where reward distributions have only finite $(1+v)$-th moments with some $v \in (0,1]$. By resorting to robust mean estimators for rewards, we first propose two frameworks for heavy-tailed MDPs, i.e., one is for value iteration and another is for policy optimization. Under each framework, we consider both joint differential privacy (JDP) and local differential privacy (LDP) models. Based on our frameworks, we provide regret upper bounds for both JDP and LDP cases and show that the moment of distribution and privacy budget both have significant impacts on regrets. Finally, we establish a lower bound of regret minimization for heavy-tailed MDPs in JDP model by reducing it to the instance-independent lower bound of heavy-tailed multi-armed bandits in DP model. We also show the lower bound for the problem in LDP by adopting some private minimax methods. Our results reveal that there are fundamental differences between the problem of private RL with sub-Gaussian and that with heavy-tailed rewards.

==> rebuttal.tex <==

\textbf{General response: An attempt for a tighter lower bound}

We thank the reviewers for their interest and constructive insights on obtaining a tighter lower bound (i.e., depending on the number of episodes). In fact, we have already tried to adapt the standard approach for RL lower bound when we prepared our submission. However, there exists one key challenge: it seems difficult to enlarge the lower bound by a factor of $H$ while not violating the assumption of heavy-tailed rewards. 

In the following, we are happy to share more details on our attempt.
%\xingyu{leave it to Yulian to fill in. Also, try to clean it. More importantly, ensure all the equations can be displayed correctly on openreview}

\textbf{An attempt for constructing non-private MDPs instances with multiple-step heavy-tailed rewards.} Let us first consider the $3$-state case to gain the key intuition. Specifically,  we consider the following construction. The Initial state (I), the Good state (G), and the Bad state (B). The starting state is always $s_1 = I$. We also assume that $\mathbb{P}({ s_2 = G| s_1 = I, a_1 = a^*}) = 2 \gamma^{1+v}$ and for any other $a \neq a^*$, $\mathbb{P}({ s_2 = G| s_1 = I, a_1 = a}) = \gamma^{1+v}$, where $\gamma^{1+v}\in (0,\frac{1}{2}]$. How about the reward for the first step? We consider the case that when the agent lands at $G$, the reward is $1/\gamma$ and when the agent lands at $B$, the reward is $0$. This ensures that $R_1(s_1 = I, a_1 = a)$ (which is a random variable) under each $a$ has bounded $(1+v)$-th moment.

For $h \ge 2$, the agent can only be at either state $B$ or state $G$, and both are self-absorbing states. For the bad state $B$, the reward is always zero. For the good state $G$, the reward belongs to a heavy-tailed distribution, i.e., for any action $a$, $R_h(s_h = G, a_h = a) = 1/\gamma$ w.p. $\gamma^{1+v}$, otherwise $0$. Note that $R$ is a random variable and it has bounded $(1+v)$ moment.

Following the paper (Domingues et al., 2021), we first determine the regret of any policy $\pi$ under the MDP, denoted by $M_{a^*}$, i.e., $a^*$ is the special arm. ($M_0$ is an MDP where there is no special arm)

The expected total reward for a given episode under any policy $\pi$ is given by 
$$\mathbb{E}[\{\sum_{h=1}^H R_h(s_h,a_h)\}]= \mathbb{E}[\{R_1(s_1,a_1)\} ]+ \mathbb{E}[\{\sum_{h=2}^H R_h(s_h, a_h)\}]$$
We have the following general regret lower bound over $K$ episodes (not steps), which is the common pattern behind nearly all the lower bounds
   $$ R(T) \ge \text{Reg} \cdot \left(1 - \sqrt{\frac{K}{A} \cdot \text{KL}}\right),$$
where the $\text{Reg}$ term captures the maximum regret (i.e., the largest difference in total expected reward), while the $\text{KL}$ term captures the similarity. Those two are conflicting with each other and all we need is to find the best balance. 

With the above hard instance construction, we can bound the two terms.
For the $\text{KL}$ term, by standard argument, we have 
\begin{align}
    \text{KL} \approx KL(\gamma^{1+v} || 2\gamma^{1+v}) \approx  \frac{\gamma^{1+v}}{(1-2\gamma^{1+v})}
\end{align}

For the $\text{Reg}$ term, we have 
$$
    \text{Reg} \approx K\cdot \left(\gamma^{1+v} \cdot \frac{1}{\gamma} +  \gamma^{1+v} \cdot (H-1) \cdot \gamma^v\right) \quad \quad \quad \quad (1)
$$

\textbf{What's the issue?} 

The issue is that we \textbf{hope} to get that $\text{Reg}$ is on the order of $K H \gamma^v$, then with choice of $\gamma = \left(\frac{A}{K+2A}\right)^{\frac{1}{1+v}}$, we can achieve the lower bound as (assume $K \ge A$)
$$
    R(T) \ge H \cdot K^{\frac{1}{1+v}} A^{\frac{v}{1+v}},
$$
which successfully enlarges the lower bound of heavy-tailed MAB by a factor of $H$.

However, by (1), we cannot get what we want for the $\text{Reg}$ term. The key problem lies in the second term in (1), which is too small. We would like to leave this as an open problem.




\textbf{Reviewer zYHM}

Thanks for your comments. We appreciate your positive comments on our exposition of the problem and theoretical results. In the following, we recap your comments and provide a detailed response to each of them. We hope our response will help you become more favorable of our paper.

\textbf{Challenges.} Thanks for the question and we would like to highlight the challenges below for plugging in private confidence bound to UCB. Besides, we also would like to refer you to Appendix A (Related Work and Challenges Section) for more challenges of this work.
\begin{itemize}
    \item  The challenge first comes from the private error due to heavy-tailed rewards is quite different from the case of the bounded reward. In detail, it's notable that $E_{\epsilon, \delta,k, 2}$ in Lemma 1 and Lemma 2 is proportional to the truncation threshold $B_k$ where $B_k$ is a non-decreasing function of $k$ and is related to privacy for balance the biased-variance trade-off and privacy-utility trade-off. Thus, we need to take different forms of $B_k$ for different algorithmic frameworks and different DP models when we plug in the private confidence bound to different UCB algorithms (See the different values of $B_k$ in Theorem 2 for UCBVI in JDP, Theorem 3 for UCBVI in LDP,  Theorem 5 for UCBPO in JDP and Theorem 6 for UCBPO in LDP.)
    \item Due to $B_k$, our DP noise allocation method is totally different from it of the bounded reward case. See our discussions in lines 232-256 and the second point in our challenge discussion in Appendix A (lines 655-674). 
    \item From the proof technical view, the analysis of the heavy-tailed case is more complicated than the bounded reward case. We cannot directly use the proof techniques for the bounded case. Due to the heavy-tailed rewards, we developed new analysis tools and proof techniques. And we think these tools can also be used in other RL problems. 
\end{itemize}


\textbf{A tighter lower bound.} We hope our general response above may have helped to 
shed light on this sharp question.


\textbf{Reviewer UVAb.}

Thanks for your appreciation of our work. We are glad to hear that you think we have made substantial contributions and support the acceptance of our paper. In the following, we recap your questions and provide a detailed response. 


\textbf{A tighter lower bound.} We hope our general response above may have helped to 
shed light on this valuable question.


\textbf{Further improvement on $H$.} Thanks for pointing out this nice related work. We believe the techniques in [1] could be applied under heavy-tailed rewards to improve the first term of regret upper bounds. We make the discussions as follows and will add the discussions in our next version.
\begin{itemize}
    \item For JDP, we achieve regret bound for Private-Heavy-UCBVI of $  \tilde{O}(\sqrt{SAH^3T} + \frac{S^2AH^3}{\epsilon} + u^{\frac{1}{1+v}}(\frac{SAH^2}{\epsilon})^{\frac{v}{1+v}}T^{\frac{1}{1+v}})$ in Theorem 2 for heavy-tailed rewards case. Compared with the regret bound of $\widetilde{O}(\sqrt{S A H^2 T}+S^2 A H^3 / \epsilon)$ given by [1] under JDP by adopting DP-UCBVI for bounded rewards, the difference of the first term comes from the type of bonus since [1] adopts Bernstein type but we use Hoeffding type. And the additional third term in our bound is due to the heavy-tailed nature of the rewards.
    
    \item For LDP, we derive regret bound of $\tilde{O}(\sqrt{SAH^3T}  + \frac{S^2A\sqrt{H^5T}}{\epsilon} + u^{\frac{1}{(1+v)}}(\frac{H^3SA}{\epsilon^2})^{\frac{v}{2(1+v)}}T^{\frac{2+v}{2(1+v)}})$ in Theorem 3 based on value-iteration method for heavy-tailed rewards case. Compared with the bound of $\widetilde{O}\left(\sqrt{S A H^2 T}+S^2 A \sqrt{H^5 T} / \epsilon\right)$ provided by [1] under LDP based on value iteration method for bounded rewards case, except for the difference in the first term as in JDP, the third term is different due to heavy-tailed rewards and the noise magnitude of private count is $\sqrt{k}$ for LDP.
\end{itemize}


\textbf{Reviewer WejM}

Thanks for your positive comments. We will follow your constructive suggestion to include more discussion on our technical contributions in the main paper. In the following, let us provide detailed answers to your two interesting questions. 

\textbf{Technical contributions.} We would
like to highlight our technical contributions.
\begin{itemize}
    \item Unlike the techniques to achieve privacy guarantees in private MAB with heavy-tailed rewards where DP mechanism can be directly used on truncated rewards such as [TWZW22], now we not only need to protect the rewards but also need to protect the transition probability by adopting the privacy mechanisms on counts. 

    
    \item Unlike the techniques in private MDP with bounded rewards case where the private bonus can be directly decomposed to the sum of the mean estimation error and private count error, the heavy-tailed case needs to set different truncation threshold values of $B_k$ to balance the biased-variance trade-off and privacy-utility trade-off  (See the different values of $B_k$ in Theorem 2 for UCBVI in JDP, Theorem 3 for UCBVI in LDP,  Theorem 5 for UCBPO in JDP and Theorem 6 for UCBPO in LDP.)

   \item Based on heavy-tailed rewards setting, the proof techniques for deriving upper bounds and lower bounded are quite different from the bounded case. For upper bounds, except for taking care of the balance of the biased-variance trade-off and privacy-utility trade-off for deriving the upper bounds, we also prove some new basic inequalities for heavy-tailed distributions, such as proofs of Lemma 12, Lemma 17, Lemma 21 which can be used for other RL models. For lower bounds, except for proof techniques, the constructions of transition probabilities and rewards are totally different from the previous bounded instances.
\end{itemize}


\textbf{Lower bound.} Yes, you are correct since MAB can be treated as a special case of general RL with $S=1$ and $H=1$. On the other hand, it is worth noting that for general RL, one is often interested in the dependence on $S$ and $H$. In general, the RL problem is more involved than MABs due to additional state transitions. 

\textbf{LDP vs. JDP.} In general, in the LDP model where the privatizer is at each user's local side, the neighboring input dataset of the privatizer is any pairs of data, e.g., two trajectories in our RL setting. On the other hand, for JDP, the neighboring dataset of the private mechanism are two neighboring user sequences, e.g., for RL, it means replacing one particular user for any episode. Note that, since this can be replaced by any other user, it also includes all possible different trajectories. It is also notable that our current LDP definition is widely used in existing private RL literature, see [GVCM21,CZ22,QW23].

[TWZW22] Tao, Youming, Yulian Wu, Peng Zhao, and Di Wang. "Optimal rates of (locally) differentially private heavy-tailed multi-armed bandits." In International Conference on Artificial Intelligence and Statistics, pp. 1546-1574. PMLR, 2022.
    
[GVCM21] Garcelon, Evrard, Vianney Perchet, Ciara Pike-Burke, and Matteo Pirotta. "Local differential privacy for regret minimization in reinforcement learning." Advances in Neural Information Processing Systems 34 (2021): 10561-10573.

[CZ22] Chowdhury, Sayak Ray, and Xingyu Zhou. "Differentially private regret minimization in episodic markov decision processes." In Proceedings of the AAAI Conference on Artificial Intelligence, vol. 36, no. 6, pp. 6375-6383. 2022.

[QW23] Qiao, Dan, and Yu-Xiang Wang. "Near-Optimal Differentially Private Reinforcement Learning."  International Conference on Artificial Intelligence and Statistics, 2023.


\yulian{google doc link: \url{https://docs.google.com/document/d/18Sm7LyUL_Gn5Ck_h9DBUFMprASB71Zh9_8jxAUR1Hyw/edit?usp=sharing}}
